TIGER: A Generating-Then-Ranking Framework for Practical Python Type Inference

Python's dynamic typing system offers flexibility and expressiveness but can lead to type-related errors, prompting the need for automated type inference to enhance type hinting. While existing learning-based approaches show promising inference accuracy, they struggle with practical challenges in comprehensively handling various types, including complex generic types and (unseen) user-defined types. In this paper, we introduce TIGER, a two-stage generating-then-ranking (GTR) framework, designed to effectively handle Python's diverse type categories. TIGER leverages fine-tuned pre-trained code models to train a generative model with a span masking objective and a similarity model with a contrastive training objective. This approach allows TIGER to generate a wide range of type candidates, including complex generics in the generating stage, and accurately rank them with user-defined types in the ranking stage. Our evaluation on the ManyTypes4Py dataset shows TIGER's advantage over existing methods in various type categories, notably improving accuracy in inferring user-defined and unseen types by 11.2% and 20.1% respectively in Top-5 Exact Match. Moreover, the experimental results not only demonstrate TIGER's superior performance and efficiency, but also underscore the significance of its generating and ranking stages in enhancing automated type inference.

==> src/discussion.tex <==
\section{Discussion}\label{sec:disucss}

==> src/intro_copy.tex <==
%% Background
Python, a widely used and versatile programming language, is lauded for its dynamic typing system, a feature that allows for code that is both adaptable and expressive. However, this dynamism can give rise to complications, notably concerning code comprehensibility, maintainability, and type-related errors~\cite{pldi/AllamanisBDG20,icse/MirLPG22,corr/abs-2307-09163}\todo{more citations}. In acknowledgment of these challenges, the Python Enhancement Proposal (PEP) 484~\cite{PEP484} was introduced as a significant stride in enhancing Python's type hinting system. PEP 484 advocates the inclusion of type hints in Python code, thereby promoting an enhancement in code quality and facilitating tooling support~\cite{Mypy,Pyre,Pyright,pytype}, including static type checking, without forsaking Python's dynamic essence.

%% Existing Approaches
Manual type annotation can be a time-consuming and error-prone endeavor, particularly within large and often complex codebases. As a remedy, there is a growing impetus to employ automated methods for inferring variable types, function arguments, and return values through contextual analysis. Notably, these type inference methods encompass rule-based and learning-based approaches.\todo{Give a more consistent classification...}
Rule-based inference approaches~\cite{Mypy,Pyre,Pyright,pytype}, which rely on predefined patterns and rules to infer types, hold promise for effective type hinting, yet they encounter \emph{practical} challenges in offering comprehensive coverage for all scenarios~\cite{sigsoft/JesseDA21,corr/abs-2307-09163}. On the other hand, learning-based approaches leverage techniques, such as supervised training~\cite{pldi/AllamanisBDG20,sigsoft/PradelGL020,sigsoft/JesseDA21,icse/MirLPG22}, cloze-style task formulation~\cite{emnlp/0034WJH21,acl/GuoLDW0022,iclr/FriedAL0WSZYZL23,kbse/HuangYXX0022}, and zero-/few-shot generative approaches~\cite{corr/abs-2307-09163} based on large language models (LLMs), to exhibit broader coverage and enhanced inference accuracy. 

%% Challenges
However, the learning-based approaches also confront two main \emph{practical challenges}.
\emph{The first challenge stems from the handling of previously unseen user-defined types.} While certain approaches incorporate user-defined types through open type vocabularies~\cite{pldi/AllamanisBDG20,sigsoft/PradelGL020,sigsoft/JesseDA21,icse/MirLPG22,emnlp/0034WJH21,acl/GuoLDW0022,iclr/FriedAL0WSZYZL23} or type-inclusive prompts~\cite{corr/abs-2307-09163}, they grapple with accuracy limitations, primarily due to issues related to the generalizability and robustness of the learned representations or prompts. Notably, strategies like the formulation of type inference as a cloze-style task~\cite{emnlp/0034WJH21,acl/GuoLDW0022,iclr/FriedAL0WSZYZL23,kbse/HuangYXX0022} may face difficulties with unfamiliar user-defined types, as they may fail to capture the features of the types and their relationship with the code context. Similarly, even the recent state-of-the-art few-shot generative approach, \typegen~\cite{corr/abs-2307-09163}, contends with accuracy reductions when comparing multiple (unfamiliar) user-defined types and distinguishing correct ones.
% \emph{The second challenge pertains to the inference cost and scalability of the LLM-based generative approaches.} Leading LLM-based generative inference approaches, such as \typegen~\cite{corr/abs-2307-09163}, rely on external APIs like OpenAI's~\cite{OpenAIAPI} for interaction with LLMs such as \texttt{gpt-3.5} and \texttt{gpt-4}, incurring significant time overhead and financial expenses, which may limit their scalability. Moreover, to bolster inference accuracy, these approaches often employ mechanisms such as self-consistency and voting~\cite{iclr/0002WSLCNCZ23}, necessitating multiple queries to LLMs, further amplifying the computational and financial burden.

%% Strategy
To address the challenges, we propose the adoption of a two-stage \gtr strategy, as depicted in Figure~\ref{fig:strategy}, to enhance the practicality of type inference for Python. Within the \emph{generating} stage, this strategy seeks to encompass different candidate types, including elementary types (\eg ``UUID'') and generic types (\eg ``Union[str,int]''). Subsequently, in the \emph{ranking} stage, project-specific, and potentially unfamiliar user-defined types (\eg ``IDMap'' and ``IDMapKey'') are considered and ranked alongside the generated candidates. To achieve this, we formulate the \emph{generating} stage as a cloze-style task, involving the infilling of type placeholders (\eg ``\orangebox{\texttt{<TYPE>}}'' in Figure~\ref{fig:strategy}) in a type-missed function; while in the \emph{ranking} phase, the sorting of types is based on their contextual relevance with the type-missed function. This two-stage strategy allows for the inclusion of diverse candidate types and facilitates a more effective comparison among them. Moreover, by leveraging relatively lightweight models such as CodeT5 (with 220 million parameters in its base version)~\cite{emnlp/0034WJH21}, this approach is more scalable compared to the LLM-based approaches like \typegen.

\begin{figure}
    \includegraphics[width=1.0\columnwidth]{imgs/strategy.pdf}
    \caption{Two-Stage \gtr Inference Strategy}
    \label{fig:strategy}
\end{figure}

%% Approach
We introduce \app, a novel approach for Python type inference built upon the two-stage strategy. To support the \gtr strategy, \app first trains a generation model and a similarity model by fine-tuning code pre-trained models, specifically CodeT5~\cite{emnlp/0034WJH21}, using annotated Python functions. 
For training the generation model, \app masks the variable types in annotated functions, replacing them with type placeholders to create type-missed functions. These type-missed functions, along with the corresponding expected types, are then employed to fine-tune a CodeT5 model, guided by a generative span masking objective~\cite{emnlp/0034WJH21}, which instructs the model to generate suitable types to fill the placeholders.
In the case of similarity model training, \app analyzes import statements to identify available user-defined types for the type-missed functions, which are combined with the types generated by the generation model to form a set of candidate types. \app then utilizes a contrastive training objective~\cite{icml/ChenK0H20,corr/abs-1807-03748,nips/OordVK17,cvpr/He0WXG20} to fine-tune a CodeT5 model, instructing it to distinguish expected types from all candidate types based on their contextual similarities to the type-missed functions.
With the trained generation model and similarity model, \app performs type inference for a given type-missed function containing type placeholder, following the \gtr strategy, which involves generating candidates and then ranking them alongside available user-defined types.


%% Evaluation
We conduct extensive experiments to evaluate the inference effectiveness of \app from different perspectives, using the widely used ManyTypes4Py dataset. The results show that \app significantly outperforms baseline approaches in terms of overall inference accuracy, different categories of variables (\eg function arguments), and different categories of type annotations (\eg unseen user-defined types). Furthermore, the ablation study confirms the contributions of the two-stage strategy, especially for addressing the challenge in handling previous unseen user-defined types. \todo{give the detailed experimental results...}

To summarize, this paper makes the following contributions:
\begin{itemize}
    \item A novel two-stage strategy ...
    \item ...
\end{itemize}





